Supersymmetric gauged matrix models from dimensional reduction on a sphere

It was recently proposed that N=1 supersymmetric gauged matrix models have a duality of order four - that is, a quadrality - reminiscent of infrared dualities of SQCD theories in higher dimensions. In this note, we show that the zero-dimensional quadrality proposal can be infered from the two-dimensional Gadde-Gukov-Putrov triality. We consider two-dimensional N=(0,2) SQCD compactified on a sphere with the half-topological twist. For a convenient choice of R-charge, the zero-mode sector on the sphere gives rise to a simple N=1 gauged matrix model. Triality on the sphere then implies a triality relation for the supersymmetric matrix model, which can be completed to the full quadrality.

==> pref.tex <==

\newcommand{\todo}[1]{{\bf ?????!!!! #1 ?????!!!!}\marginpar{$\Longleftarrow$}}
\newcommand{\tocite}{{[!CITE!]}\marginpar{$\Longleftarrow\Longleftarrow!!!$}}
\newcommand{\tocheck}{{[!CHECK!]}\marginpar{$\Longleftarrow\Longleftarrow!!!$}}
\newcommand{\towrite}{{[WRITING...]}\marginpar{$\Longleftarrow\Longleftarrow!!!$}}

\newcommand{\be}{\begin{equation}}
\newcommand{\ee}{\end{equation}}
\newcommand{\beq}{\begin{equation}}
\newcommand{\beql}[1]{\begin{equation}\label{#1}}
\newcommand{\eeq}{\end{equation}}
\newcommand{\ba}{\begin{array}}
\newcommand{\ea}{\end{array}}
\newcommand{\bea}{\begin{eqnarray}}
\newcommand{\beal}[1]{\begin{eqnarray}\label{#1}}
\newcommand{\eea}{\end{eqnarray}}
\newcommand{\ben}{\begin{enumerate}}
\newcommand{\een}{\end{enumerate}}
\newcommand{\bean}{\begin{eqnarray*}}
\newcommand{\eean}{\end{eqnarray*}}
\newcommand{\eref}[1]{(\ref{#1})}
\newcommand{\sref}[1]{\S\ref{#1}}
\newcommand{\tref}[1]{Table~\ref{#1}}
\newcommand{\nn}{\nonumber}
\newcommand{\pa}{\partial}
\newcommand{\oline}{\overline}
\newcommand{\bvec}{\left(\ba{c}}
\newcommand{\evec}{\ea\right)}
\newcommand{\bvset}[1]{\left\{\ba{#1}}
\newcommand{\evset}{\ea\right\}}
\newcommand{\fref}[1]{Figure \ref{#1}}
\newcommand{\btab}[1]{\begin{tabular}{#1}}
\newcommand{\etab}{\end{tabular}}
\newcommand{\diag}{\mbox{diag}}
\newcommand{\master}{\mathcal{F}^\flat}
\newcommand{\irrmaster}{{}^{\text{Irr}}\mathcal{F}^\flat}
\newcommand{\mesonic}{\mathcal{M}^{mes}}

\def \Red {\pdfsetcolor{0 1 1 0}}
\def \Green {\pdfsetcolor{1 0 1 0}}
\def \Blue {\pdfsetcolor{1 1 0 0}}
\def \Black {\pdfsetcolor{0 0 0 1}}

\newcommand{\BC}{\mathbb{C}}
\newcommand{\BR}{\mathbb{R}}
\newcommand{\BZ}{\mathbb{Z}}
\newcommand{\comment}[1]{}
\newcommand{\CF}{{\cal F}}
\newcommand{\CM}{{\cal M}}
\newcommand{\CW}{{\cal W}}
\newcommand{\CN}{{\cal N}}
\newcommand{\CB}{{\cal B}}
\newcommand{\IP}{\mathbb{P}}
\newcommand{\IC}{\mathbb{C}}
\newcommand{\vev}[1]{\langle #1 \rangle}
\def\tQ{\widetilde{Q}}
\def\tB{\widetilde{B}}

\newcommand{\ud}{\mathrm{d}}
\newcommand{\bull}{$\bullet\ $}
\newcommand{\CP}{\mathbb P}

\newcommand{\PE}{\mathrm{PE}}
%\newcommand{\PE}[1]{\mathrm{PE}\left[#1\right]}
\newcommand{\PL}{\mathrm{PL}}
%\newcommand{\PL}[1]{\mathrm{PL}\left[#1\right]}

\newcommand{\mqcd}{\CM_{(N_f,N_c)}}

\newtheorem{theorem}{\bf Theorem}
\def\thetheorem{\thesection.\arabic{theorem}}
\newtheorem{conjecture}[theorem]{\bf Conjecture}
\newtheorem{observation}[theorem]{\bf Observation}
\newtheorem{lemma}[theorem]{\bf Lemma}

\def\theequation{\thesection.\arabic{equation}}
\newcommand{\setall}{\setcounter{equation}{0}
        \setcounter{theorem}{0}}
\newcommand{\setequation}{\setcounter{equation}{0}}


\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{corollary}[theorem]{Corollary}

\newenvironment{proof}[1][Proof]{\begin{trivlist}
\item[\hskip \labelsep {\bfseries #1}]}{\end{trivlist}}
\newenvironment{definition}[1][Definition]{\begin{trivlist}
\item[\hskip \labelsep {\bfseries #1}]}{\end{trivlist}}
\newenvironment{example}[1][Example]{\begin{trivlist}
\item[\hskip \labelsep {\bfseries #1}]}{\end{trivlist}}
\newenvironment{remark}[1][Remark]{\begin{trivlist}
\item[\hskip \labelsep {\bfseries #1}]}{\end{trivlist}}

\newcommand{\qed}{\nobreak \ifvmode \relax \else
      \ifdim\lastskip<1.5em \hskip-\lastskip
      \hskip1.5em plus0em minus0.5em \fi \nobreak
      \vrule height0.75em width0.5em depth0.25em\fi}

